Deterministic Memory Abstraction and Supporting Multicore System Architecture

Poor time predictability of multicore processors has been a long-standing challenge in the real-time systems community. In this paper, we make a case that a fundamental problem that prevents efficient and predictable real-time computing on multicore is the lack of a proper memory abstraction to express memory criticality, which cuts across various layers of the system: the application, OS, and hardware. We, therefore, propose a new holistic resource management approach driven by a new memory abstraction, which we call Deterministic Memory. The key characteristic of deterministic memory is that the platform - the OS and hardware - guarantees small and tightly bounded worst-case memory access timing. In contrast, we call the conventional memory abstraction as best-effort memory in which only highly pessimistic worst-case bounds can be achieved. We propose to utilize both abstractions to achieve high time predictability but without significantly sacrificing performance. We present deterministic memory-aware OS and architecture designs, including OS-level page allocator, hardware-level cache, and DRAM controller designs. We implement the proposed OS and architecture extensions on Linux and gem5 simulator. Our evaluation results, using a set of synthetic and real-world benchmarks, demonstrate the feasibility and effectiveness of our approach.

==> analysis-static.tex <==
\section{LRU Persistence Analysis under Deterministic Memory}

In this section we provide a sketch of how persistence analysis for
LRU fully-associative caches~\cite{LRU_analysis_book, LRU_fix,
  LRU_ferdinand} can be extended when deterministic memory at the
cache controller is implemented according to
Algorithm~\ref{alg:cacherepl}. We indicate with ``DM-LRU'' the
resulting cache policy. In this section, we only discuss \emph{must}
analysis for the single-core case, to demonstrate that it is possible
to predict cache hits that could not be classified as \emph{always
  hit} for the same control flow (process) if DM was not
used. Following the outlined approach, \emph{may} analysis could also
be extended. Persistence analysis was first introduced
in~\cite{LRU_ali, LRU_ferdinand}, and formalized in~\cite{LRU_reineke,
  LRU_analysis_book}. We reuse some of the notation
in~\cite{LRU_analysis_book}, but due to space constraints we omit a
number of details.

In this analysis framework, \emph{must} analysis is performed by
considering abstracted cache states. \emph{Must} analysis keeps track
of the upper-bound on the age of each addressable memory block. The
abstract domain $DMLru_{D+B}$ is defined as $DMLru_{D+B} :=
\mathcal{B} \rightarrow \{0, \ldots, D-1\} \times \{D, \ldots, D+B-1,
\infty\}$, where $D+B = A$, with $A$ being the associativity of the
cache, and $D$ ($B$, resp.) is the number of lines marked as
deterministic (best-effort, resp.). An abstract state $q$ is then
represented as two sets of memory blocks $q =
[\{a,b\}],[\{c\},\{d\},\{e,f\}] \in DMLru_{D+B}$. In this example, we
have $D = 1, B = 3, A = 4$. Any block with DM-LRU age greater than or
equal to D is a best-effort block. Hence, blocks $a$ and $b$ are
deterministic lines, with maximum DM-LRU age 0. On the other hand $d$
is a best-effort block with maximum DM-LRU age 2.

%% When a new memory reference is performed, the access can lead to 4
%% different cases: ($M_d$) miss on DM line, ($H_d$) hit on DM line,
%% ($M_b$) miss on best-effort line, ($H_d$) hit on best-effort line.

The update abstract transformer $U_{D}$ for a deterministic memory
access $a$ can be defined as follows:

{\scriptsize
\begin{multline}
  U_{D}(q, a) := D' \leftarrow
  \begin{cases}
    D + 1 &:= D < A-1 \land q(a) \ge D\\
    D     &:= D = A \lor q(a) < D\\
  \end{cases},
  B' \leftarrow
  \begin{cases}
    B - 1 &:= D < A-1 \land q(a) \ge D\\
    B     &:= D = A \lor q(a) < D\\
  \end{cases},\\
  \lambda b. 
  \begin{cases}
    0         &:= b = a\\
    q(b)      &:= b \neq a \land q(b) < D \land q(b) \ge q(a) \\
    q(b)+1    &:= b \neq a \land q(b) < D \land q(b) < q(a) \land q(b) < D'-1\\
    \infty    &:= b \neq a \land q(b) < D \land q(b) < q(a) \land q(b) \ge D'-1\\
    q(b)      &:= b \neq a \land q(b) \ge D \land q(a) < D\\
    q(b)      &:= b \neq a \land q(b) \ge D \land q(b) \ge q(a)\\
    q(b)+1    &:= b \neq a \land q(b) \ge D \land q(b) < q(a) \land q(b) < A-1\\
    \infty    &:= b \neq a \land q(b) \ge D \land q(b) < q(a) \land q(b) \ge A-1\\
  \end{cases}
  \label{eq:u_d_transf}
\end{multline}
}

Where $D'$ ($B'$, resp.) is the new value of $D$ ($B$, resp.) after
the update. Similarly, the update abstract transformer $U_{B}$ for a
best-effort memory access $a$ can be defined as follows:

{\scriptsize
\begin{equation}
  U_{B}(q, a) :=
  \lambda b. 
  \begin{cases}
    D         &:= b = a\\
    q(b)      &:= b \neq a \land q(b) \ge q(a) \\
    q(b)+1    &:= b \neq a \land q(b) < q(a) \land q(b) < A-1\\
    \infty    &:= b \neq a \land q(b) < q(a) \land q(b) \ge A-1\\
  \end{cases}
\end{equation}
}

The join abstract transformer remains almost identical to what used in
traditional LRU \emph{must} analysis~\cite{LRU_reineke,
  LRU_analysis_book}: the joined state will contain only the blocks in
the intersection of the joining states, each with the maximum age in
any of the two states. The only difference is that $D$ is taken as the
maximum between the value of $D$ in the joining states. $B$ for the
new state is then computed as $A-D$.

To clarify update and join operations, consider the abstract state $q
= [\{a,b\}],[\{c\},\{d\},\{e,f\}]$, where $D = 1$.  Assume that
deterministic block $d$ is accessed, which is currently cached as
best-effort (this can happen after a context-switch). First, the value
of $D'$ ($B'$, resp.) is computed as $D' = D+1$ ($B' = B - 1$, resp.);
next, $\{a,b\}$ both satisfy the third condition in the age
transformation of $U_{D}$ (Equation~\ref{eq:u_d_transf}); block $c$
satisfies the seventh condition; $d$ the first; and $\{e,f\}$ the
sixth. The resulting updated abstract state is: $q' =
[\{d\},\{a,b\}],[\{c\},\{e,f\}]$. If we were to join $q$ with $q'$,
the resulting state would be $q'' = [\{\},\{a,b\}],[\{c,d\},\{e,f\}]$.

\begin{figure}
  \centering
  \includegraphics[width=.9\textwidth]{figs/dm_lru}
  \caption{An example of \emph{must} analysis under DM-LRU (orange
    states), compared to traditional LRU (blue states). If $a$ and $f$
    are marked as DM, they can be classified as \emph{always hit} under
    DM-LRU.}
  \label{fig:dm_lru}
\end{figure}

We now demonstrate how this analysis can be applied to a simple
control-flow graph. The following example yields an important
conclusions: there exist instances where it is not possible to predict
any cache hit with traditional LRU, while under DM-LRU it is possible
to predict some cache hits. For our example, we consider a cache with
$A = 4$. The initial state is $[\{\},\{\},\{\},\{\}]$ and
$[~],[\{\},\{\},\{\},\{\}]$ for LRU and DM-LRU, respectively. The
progress of the analysis is depicted in Figure~\ref{fig:dm_lru}. As
shown in the example, blocks $a$ and $f$ can be classified as
\emph{persistent} (i.e. always hit after the first miss) under DM-LRU,
while they cannot be classified as \emph{always hit} if traditional LRU
is used.


==> eval-analysis.tex <==
\subsection{Analytic WCRT Comparison}

\begin{figure} [h]
  \centering
  \includegraphics[width=0.48\textwidth]{figs/slowdown_analytic.pdf}
  \caption{Analytical worst-case slowdown.}
  \label{fig:slowdown-analytic}
\end{figure}

In this subsection, we analytically compare worst-case response times
(WCRTs) the real-time benchmarks used in Section~\ref{sec:evaluation},
using the timing analysis method described above.

For this comparison, we use profiled L1 miss counts of the
benchmarks. We then compute each task's WCRT by adding its solo WCET
and the worst-case inter-core interference delay, $I$. 
For NoP, we assume every L1 miss would suffer
$RD^{bm}$, the worst-case inter-core delay of a best-effort memory
request. For DM(H), we use Eq.~\ref{eq:interference}, which
distinguishes deterministic and best-effort L1 misses. Lastly, for
DM(A) and WP assume all L1 misses are inter-core interference free
(i.e., $I = 0$). Figure~\ref{fig:slowdown-analytic} shows the
calculated WCRTs of the benchmarks. In this figure, we set
$RD^{bm}=50$ and $RD^{dm}=0$ (in cycles).



==> eval-best-effort.tex <==
\subsection{Additional Results for Best-effort Tasks} \label{subsec:ext-best-effort}

\begin{figure} [h]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\linewidth]{figs/cache-occ-3bzip2.pdf}
        \caption{The percentage of total cache space occupied by \emph{bzip2} running on 3 cores.}
        \label{fig:bzip2-benefit2_a}
    \end{subfigure}
    \vfill
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\linewidth]{figs/hit-rate-cr-3bzip2.pdf}
        \caption{Average hit rate for \emph{bzip2} running on 3 cores.}
        \label{fig:bzip2-benefit2_b}
    \end{subfigure}

    \caption{Cache usage and hit rate of \emph{bzip2}.
    The real-time task is running Core 3, and
    three instances of \emph{bzip2} are running on Core 0 through 2.}
    \label{fig:bzip2-benefit2}
\end{figure}

\begin{figure} [h]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\linewidth]{figs/cache-occ-1mcf.pdf}
        \caption{The percentage of cache space occupied by \emph{mcf}.}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\linewidth]{figs/hit-rate-cr-1mcf.pdf}
        \caption{\emph{mcf} hit rate.}
    \end{subfigure}
    \vfill
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\linewidth]{figs/cache-occ-3mcf.pdf}
        \caption{The percentage of total cache space occupied by \emph{mcf} running on 3 cores.}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\linewidth]{figs/hit-rate-cr-3mcf.pdf}
        \caption{Average hit rate for \emph{mcf} running on 3 cores.}
    \end{subfigure}

    \caption{Cache usage and hit rate of \emph{mcf} for two
    different scenarios: 1) \emph{mcf} is running on one core, and 3 instances of the
    real-time task are running on rest of the cores (figures (a) and (b));
    2) the real-time task is running on one core, and three instances of 
    \emph{mcf} are running on the rest of the cores (figures (c) and (d)).}
    \label{fig:mcf-benefit}
\end{figure}

Figure~\ref{fig:bzip2-benefit2_a} shows the result for Scenario~2
(see \ref{subsec:best-effort}).
As it can bee seen, three instances of bzip2 occupy 75\% of
cache space in WP (each gets 25\%). To calculate the cache space each
\emph{bzip2} occupies in DM(H) and DM(A), the numbers in
Figure~\ref{fig:bzip2-benefit2_a} must be divided by 3.
By doing this calculation, we can see that each \emph{bzip2}
occupies less cache space compared to what has been observed in Scenario~1
(Figure \ref{fig:bzip2-benefit_a}). This results in a smaller hit rate improvement 
compared to Scenario~1, as can be observed by comparing Figure~\ref{fig:bzip2-benefit_b} 
and Figure~\ref{fig:bzip2-benefit2_b}.

Figure~\ref{fig:mcf-benefit} shows the result for \emph{mcf}. By comparing
this figure to figures \ref{fig:bzip2-benefit} and \ref{fig:bzip2-benefit2},
we can observe that the amount of cache space that \emph{mcf} and \emph{bzip2}
are allowed to occupy is the same. This means that, although cache space occupation 
increase from WP to DM(H) or DM(A) is the same
for both benchmarks, \emph{bzip2} benefits more from the additional space in terms of hit rate.




==> eval-ext.tex <==

\subsection{4MB Cache}
In order to examine the effect of cache size on the performance of our method, we repeat
the same experiment with 4Mb cache size. We also set the total working set size of the co-runners
to be equal to the new cache size. The can observe almost the same behavior for number misses and the slowdown
in Figures~\ref{fig:missrate-4mb} and \ref{fig:slowdown-4mb} like the 2MB cache, though, the slowdown is less 
in the case of the 4MB cache. The percent of the private partition utilization by the target benchmark is decreased
since now there is twice more space is dedicated as the private partition (figure~\ref{fig:dm-util-4mb}).
Consequently, some the co-runners (e.g. mser and sift) are gaining more throughput improvement as it can be seen
in figure~\ref{fig:cr-imprv-4mb}.

\begin{figure} [h]
  \centering
  \includegraphics[width=0.45\textwidth]{figs/miss-rate2-4mb.pdf}
  \caption{Normalized numbers of L2 misses for 4MB cache.}
  \label{fig:missrate-4mb}
\end{figure}


\begin{figure} [h]
  \centering
  \includegraphics[width=0.45\textwidth]{figs/slowdown2-4mb.pdf}
  \caption{Slowdown (with respect to the solo run) for 4MB cache.}
  \label{fig:slowdown-4mb}
\end{figure}

\begin{figure} [h]
  \centering
  \includegraphics[width=0.5\textwidth]{figs/dm-util-4mb.pdf}
  \caption{Private partition utilization of the target benchmark for 4MB cache.}
  \label{fig:dm-util-4mb}
\end{figure}

\begin{figure} [h]
  \centering
  \includegraphics[width=0.5\textwidth]{figs/cr-imprv-4mb.pdf}
  \caption{Co-runners throughput improvement over way partitioned method for 4MB cache.}
  \label{fig:cr-imprv-4mb}
\end{figure}


\subsection{SD-VBS with SQCIF Input and 2Mb Cache}
Another factor that must be studied is the effect of the working set size of the target benchmark.
In order to do this, we examined the change the input size of the SD-VBS benchmark to be SQCIF.
Figures~\ref{fig:missrate-sqcif-2mb} and \ref{fig:slowdown-sqcif-2mb} are proving that the deterministic
memory can guarantee the number of misses in the shared cache and the slowdown in the presence of
co-runners running on the other cores. Since the target benchmark is using more of the private partition
in this case (figure~\ref{fig:dm-util-sqcif-2mb}), less throughput improvement improvement is observed 
by the co-runners in figure~\ref{fig:cr-imprv-sqcif-2mb}.

\begin{figure} [h]
  \centering
  \includegraphics[width=0.45\textwidth]{figs/miss-rate2-sqcif-2mb.pdf}
  \caption{Normalized numbers of L2 misses for 2MB cache and SQCIF input.}
  \label{fig:missrate-sqcif-2mb}
\end{figure}


\begin{figure} [h]
  \centering
  \includegraphics[width=0.45\textwidth]{figs/slowdown2-sqcif-2mb.pdf}
  \caption{Slowdown (with respect to the solo run) for 2MB cache and SQCIF input.}
  \label{fig:slowdown-sqcif-2mb}
\end{figure}

\begin{figure} [h]
  \centering
  \includegraphics[width=0.5\textwidth]{figs/dm-util-sqcif-2mb.pdf}
  \caption{Private partition utilization of the target benchmark for 2MB cache and SQCIF input.}
  \label{fig:dm-util-sqcif-2mb}
\end{figure}

\begin{figure} [h]
  \centering
  \includegraphics[width=0.5\textwidth]{figs/cr-imprv-sqcif-2mb.pdf}
  \caption{Co-runners throughput improvement over way partitioned method for 2MB cache and SQCIF input.}
  \label{fig:cr-imprv-sqcif-2mb}
\end{figure}


==> problem.tex <==
\section{Real-Time Cache Management Problem} \label{sec:problem}
% deterministic memory abstraction. why? 
% - memory centric resource management
%   OS and hardware can manage memory at the granularity of a page. 
%     OS page allocation, hardware cache-line allocation, dram
%     bank allocation, and dram controller request scheduling. 

Much research has been done in the real-time systems community on
how to manage shared caches to achieve predictable timing.
A typical set-associative cache is organized in sets and ways and can
be partitioned using OS-level
page-coloring~\cite{wolfe1994software,liedtke1997controlled},  
way-based partitioning on some supported
hardware~\cite{ward2013ecrts,intelcat},
or a combination of both~\cite{kim2016attacking}.
Using these partitioning mechanisms, the basic approach is to assign
dedicated cache space for each real-time task so that its cache
contents cannot be evicted by other tasks' cache accesses.

However, task-based partitioning approaches result in poor resource
utilization because the cache space dedicated to a task cannot be
utilized by other tasks. While careful allocation
strategies~\cite{chisholm2015rtss,ward2013ecrts} that assign the
minimum amount of cache space necessary for each real-time task can
reduce the amount of waste to a certain degree, as the number of
real-time tasks increase, viable cache space will eventually run out
and much of the reserved space will be under utilized. The problem is
further compounded by the fact that partitioning can not be done at a
fine granularity because most existing mechanisms---page coloring and
way partitioning---support only a small number of coarse-grained
cache partitions.

Kim et al. partly mitigated the problem by core-based cache
partitioning.
%% through a coordinated cache
%% management scheme that combines \emph{cache reservation} and \emph{cache
%% sharing}
~\cite{kim2013coordinated}. In their scheme, each core
reserves a dedicated cache partition, which is shared by
multiple tasks assigned to the core. Because a cache partition is
shared by multiple tasks, the approach can mitigate---to a
degree---the problem of limited number of cache partitions. 
Similarily, MC$^2$ framework also reserves dedicated per-core cache
space (ways and colors) for high criticaility
tasks~\cite{kim2016attacking}. 
However, the space efficiency of core-based partitioning strategy is
still fundamentally limited because a reserved cache space for a
core cannot be utilized by other cores---particularily those that
execute non real-time tasks---even if it is not fully utilized. 

%% The problem is more pronounced  when tasks within each
%% core's cache partition have very different cache space demands. 
%% For example, if a core is assigned to schedule two real-time tasks
%% where one task needs a small cache space while the other task needs a
%% relatively large amount of cache space, %% the reserved cache partition
%% %% size for the core must be based on the larger task.
%% %% Then, 
%% the reserved cache space will be \emph{under-utilized} when the
%% smaller task is scheduled on the core.
%% Although it is possible to carefully select tasks---for example,
%% co-locating tasks with similar space demands---to minimize such
%% waste, finding right tasks for the core is neither easy, because it
%% requires detailed profiling information~\cite{kim2013coordinated}, nor
%% always possible. Furthermore, a task's cache demand can change over
%% time depending on the input to the task or internal status (mode)
%% changes.

% summary of the problems.
In summary, existing task- or core-based cache partitioning approaches
suffer from inefficient cache space utilization when the reserved
space is not fully utilized by the assigned task or core, which result
in lower resource utilization and lower average throughput.
 
The low space utilization is an especially important problem given
that, for critical real-time tasks, it is a common practice to
conservatively allocate sufficient amount of resource due to the
difficulties of precisely estimating a task's working-set size. The
consequence is that much of the reserved resources would be wasted
even if there are low criticality tasks that could benefit from those
wasted resources. Unfortunately, under the existing partitioning
approaches, it is difficult, if not impossible, to reclaim these
unused reserved resources without breaking isolation guarantees that
are needed by the critical real-time tasks.

We believe this inefficiency in resource management is fundamentally
stemming from the lack of proper \emph{memory abstraction}.

%% \todo[inline]{This is all good, but somewhere it needs to be clarified
%%   why DM can overcome the mentioned limitations. (RM)}

%% % what we want.
%% Cache-lines of a RT task should not be evicted by other tasks on
%% different cores.  In particular, important cache-lines should never be
%% evicted. But not all cache lines may be important. I.e., some may be
%% okay to be evicted.
% next section.
%% In the next section, we show how deterministic memory abstraction can
%% be used to address the aforementioned problems.

%% To illustrate the challenges, consider, for example, a mixed
%% criticality system, whose taskset is composed of a large number of
%% real-time (RT) and non-real-time (NRT) tasks of varing working-set
%% sizes (WSS). We assume that the tasks are scheduled based on
%% partitioned fixed priority CPU scheduling. In such a setting, per-task
%% based cache partitioning is not effective because of a large number of
%% tasks that cannot be accommodated with only a handful of cache
%% partitions (colors or ways). Per-core based partitioning is needed but
%% then deciding which tasks to run which cores is difficult due to
%% diverse working-set sizes.




==> raw-num.tex <==
\subsection{Raw Numbers}

\begin{table}[h]
\centering
\caption{Number of Hits}
\begin{tabular}{|p{2cm}|p{1cm}|p{1cm}|p{1cm}|}
\hline
\textbf{benchmark}         & \textbf{hits}  & \textbf{accesses}  & \textbf{hit rate} \\ \hline
disparity                  & 48450          & 53447              & 0.91              \\ \hline
disparity-wp               & 53715          & 53717              & 1.00              \\ \hline
disparity-dm-h             & 53498          & 53526              & 1.00              \\ \hline
disparity-dm-all           & 53210          & 53212              & 1.00              \\ \hline
mser                       & 57799          & 73178              & 0.79              \\ \hline
mser-wp                    & 72996          & 73015              & 1.00              \\ \hline
mser-dm-h                  & 74793          & 75099              & 1.00              \\ \hline
mser-dm-all                & 73557          & 73558              & 1.00              \\ \hline
sift                       & 16104          & 30310              & 0.53              \\ \hline
sift-wp                    & 32025          & 33291              & 0.96              \\ \hline
sift-dm-h                  & 29086          & 29851              & 0.97              \\ \hline
sift-dm-all                & 46748          & 47390              & 0.99              \\ \hline
svm                        & 70903          & 73807              & 0.96              \\ \hline
svm-wp                     & 68225          & 68245              & 1.00              \\ \hline
svm-dm-h                   & 94889          & 95793              & 0.99              \\ \hline
svm-dm-all                 & 66028          & 66498              & 0.99              \\ \hline
texture\_synthesis         & 6381           & 9547               & 0.67              \\ \hline
texture\_synthesis-wp      & 8206           & 8209               & 1.00              \\ \hline
texture\_synthesis-dm-h    & 8572           & 8630               & 0.99              \\ \hline
texture\_synthesis-dm-all  & 11132          & 11136              & 1.00              \\ \hline
aifftr01                   & 148338         & 187696             & 0.79              \\ \hline
aifftr01-wp                & 168728         & 168834             & 1.00              \\ \hline
aifftr01-dm-h              & 191645         & 191898             & 1.00              \\ \hline
aifftr01-dm-all            & 184654         & 184968             & 1.00              \\ \hline
aiifft01                   & 372138         & 417717             & 0.89              \\ \hline
aiifft01-wp                & 427628         & 427783             & 1.00              \\ \hline
aiifft01-dm-h              & 445522         & 446033             & 1.00              \\ \hline
aiifft01-dm-all            & 300813         & 301114             & 1.00              \\ \hline
matrix01                   & 75646          & 92673              & 0.82              \\ \hline
matrix01-wp                & 84660          & 85600              & 0.99              \\ \hline
matrix01-dm-h              & 84045          & 85397              & 0.98              \\ \hline
matrix01-dm-all            & 93741          & 94465              & 0.99              \\ \hline
\end{tabular}
\end{table}


% \begin{table}[h]
% \centering
% \caption{Number of Misses}
% \label{my-label}
% \begin{tabular}{|p{2cm}|p{2cm}|p{2cm}|}
% \hline
%                    & \textbf{\# of L2 Accesses} & \textbf{\# of Misses NoP} \\ \hline
% disparity          & 54135                      & 9464                      \\ \hline
% mser               & 72791                      & 16716                     \\ \hline
% sift               & 29379                      & 15130                     \\ \hline
% svm                & 80416                      & 6505                      \\ \hline
% texture\_synthesis & 9266                       & 3413                      \\ \hline
% aifftr01           & 181635                     & 59801                     \\ \hline
% aiifft01           & 259748                     & 46000                     \\ \hline
% matrix01           & 94281                      & 21974                     \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[]
% \centering
% \caption{Number of Misses}
% \label{my-label}
% \begin{tabular}{|p{2cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|}
% \hline
%                    & \textbf{\# of L2 Accesses} & \textbf{\# of Misses NoP} & \textbf{\# of Misses WP} & \textbf{\# of Misses DM} & \textbf{\# of Misses DM(A)} \\ \hline
% disparity          & 54135                      & 9464                      & 1                        & 374                      & 1                           \\ \hline
% mser               & 72791                      & 16716                     & 1                        & 35                       & 1                           \\ \hline
% sift               & 29379                      & 15130                     & 54                       & 526                      & 9                           \\ \hline
% svm                & 80416                      & 6505                      & 2                        & 835                      & 220                         \\ \hline
% texture\_synthesis & 9266                       & 3413                      & 3                        & 44                       & 2                           \\ \hline
% aifftr01           & 181635                     & 59801                     & 201                      & 34543                    & 727                         \\ \hline
% aiifft01           & 259748                     & 46000                     & 185                      & 17023                    & 846                         \\ \hline
% matrix01           & 94281                      & 21974                     & 995                      & 3336                     & 2239                        \\ \hline
% \end{tabular}
% \end{table}
% 
% \begin{table}[]
% \centering
% \caption{Co-runners IPC}
% \label{my-label}
% \begin{tabular}{|p{2cm}|p{1cm}|p{1cm}|p{1cm}|}
% \hline
%                    & \textbf{IPC WP} & \textbf{IPC DM} & \textbf{IPC DM(A)} \\ \hline
% disparity          & 2.73            & 4.02            & 4.05           \\ \hline
% mser               & 2.71            & 4.37            & 4.34           \\ \hline
% sift               & 2.71            & 4.51            & 4.15           \\ \hline
% svm                & 2.72            & 2.64            & 2.58           \\ \hline
% texture\_synthesis & 2.71            & 4.58            & 4.55           \\ \hline
% aifftr01           & 2.72            & 4.55            & 4.51           \\ \hline
% aiifft01           & 2.72            & 4.52            & 4.48           \\ \hline
% matrix01           & 2.72            & 4.60            & 4.53           \\ \hline
% \end{tabular}
% \end{table}
% 
% \begin{table}[]
% \centering
% \caption{Real-time bench runtime}
% \label{my-label}
% \begin{tabular}{|p{2cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|}
% \hline
%                    & \textbf{Runtime Solo (ms)} & \textbf{Runtime NoP (ms)} & \textbf{Runtime WP (ms)} & \textbf{Runtime DM (ms)} & \textbf{Runtime DM(A) (ms)} \\ \hline
% disparity          & 0.75                       & 1.61                      & 0.749                    & 0.796                    & 0.766                       \\ \hline
% mser               & 2.47                       & 3.62                      & 2.472                    & 2.518                    & 2.518                       \\ \hline
% sift               & 3.87                       & 4.96                      & 3.881                    & 3.914                    & 3.878                       \\ \hline
% svm                & 5.36                       & 5.96                      & 5.304                    & 5.508                    & 5.4                         \\ \hline
% texture\_synthesis & 2.61                       & 2.90                      & 2.594                    & 2.614                    & 2.601                       \\ \hline
% aifftr01           & 26.80                      & 31.60                     & 26.819                   & 28.963                   & 26.894                      \\ \hline
% aiifft01           & 25.30                      & 28.81                     & 25.311                   & 26.561                   & 25.356                      \\ \hline
% matrix01           & 76.53                      & 78.61                     & 76.748                   & 76.848                   & 76.767                      \\ \hline
% \end{tabular}
% \end{table}
